Computing Divergences between Discrete Decomposable Models

There are many applications that benefit from computing the exact divergence between 2 discrete probability measures, including machine learning. Unfortunately, in the absence of any assumptions on the structure or independencies within these distributions, computing the divergence between them is an intractable problem in high dimensions. We show that we are able to compute a wide family of functionals and divergences, such as the alpha-beta divergence, between two decomposable models, i.e. chordal Markov networks, in time exponential to the treewidth of these models. The alpha-beta divergence is a family of divergences that include popular divergences such as the Kullback-Leibler divergence, the Hellinger distance, and the chi-squared divergence. Thus, we can accurately compute the exact values of any of this broad class of divergences to the extent to which we can accurately model the two distributions using decomposable models.

==> tex/_core/proof/col-complex.tex <==
\noindent
  As we have showed in Section~\ref{sec:comp-jtc}, computing $\func(\pr,\qre)$
  involves 3 steps:
  \begin{enumerate}
    \item Running the junction tree algorithm once to obtain the
    beliefs over each maximal clique in $\graphH$ with factors from
    $g\left[\pre(\xval)\right]$ and $h\left[\qre(\xval)\right]$. The
    time complexity for this step is bounded by an exponential with
    respect to the treewidth of $\graphH$.
    \item Multiplying each belief by an additional term, $L(\cdot)$,
    summing over the belief by its domain. This step is also bounded
    by an exponential with respect to the treewidth of $\graphH$.
    \item Repeating the previous step for each maximal clique in
    \glspl{dm} $\modelP$ and $\modelQ$. This results in
    multiplying the complexity of the previous step by the number of
    maximal cliques in $\modelP$ and $\modelQ$,
    $|\clis(\graph_{\pr})|$ and $|\clis(\graph_{\qr})|$ respectively.
  \end{enumerate}
  Therefore the resulting complexity is:
  \begin{align*}
    &(|\clis(\graph_{\pr})|+|\clis(\graph_{\qr})|)\cdot
    \mathcal{O}\left(2^{\text{tw}(\graphH)}\right) +
    \mathcal{O}\left(2^{\text{tw}(\graphH)}\right)\\
    &=
    \mathcal{O}\left(
      |\clis(\graph_{\pr})|+|\clis(\graph_{\qr})| \cdot
      2^{\text{tw}(\graphH)}
    \right)
  \end{align*}
  \qed

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../appendix"
%%% End:


==> tex/_core/proof/expressf1f2.tex <==
\noindent
  Recall $\func$:
  \begin{align*}
    &\func(\pr,\qr)\\
    &= \sum_{\xval\in\dom}g\left[\pr(\xval)\right] \cdot
      h\left[\qr(\xval)\right] \cdot
      L\left(g^{*}\left[\pr(\xval)\right] \cdot
      h^{*}\left[\qr(\xval)\right]\right)^{l}
  \end{align*}
  Then recall $f_1$ from Theorem~\ref{thm:ab-div-f-expr}:
  \begin{gather*}
    \begin{aligned}
    &f_{1}(\pr,\qr;a,b)=\sum_{\xval}\pr(\xval)^{a}\qr(\xval)^{b}
    \end{aligned}
    \intertext{therefore, $f_{1}(\pr,\qr;a,b)=\func(\pr,\qr)\,$  when}
    \begin{aligned}
      h(x) = x^{a} \quad g(x) = x^b
    % &h(x) = x^{a} \quad
    % &h^{*}(x) = 1\\
    % &g(x) = x^{b}\quad
    % &g^{*}(x) = 1
    \end{aligned}\\
    l=0 \implies L,g^{*},h^{*} \text{ are irrelevant}
    %L_{b}(x) = L_{1}(x) = 1
  \end{gather*}
  Also recall $f_2$ from Theorem~\ref{thm:ab-div-f-expr}:
  \begin{gather*}
    \begin{aligned}
    &f_{2}(\pr,\qr;a,b,c,d)
    =\sum_{\xval}\pr(\xval)^{a}\qr(\xval)^{b}
    \ln \left(\pr(\xval)^{c}\qr(\xval)^{d}\right)
    \end{aligned}
    \intertext{therefore, $f_2(\pr,\qr;a,b,c,d)=\func(\pr,\qr)$ when}
    \begin{aligned}
    &h(x) = x^{a} \quad
    &h^{*}(x) = x^{c}\\
    &g(x) = x^{b}\quad
    &g^{*}(x) = x^{d}\\
    \end{aligned}\\
    l=1 \quad L(x) = \ln x
  \end{gather*}
  \qed
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../estimating-divergences"
%%% End:

